The Impact of Research Funding on Knowledge Creation and Dissemination: A study of SNSF Research Grants

This study investigates the impact of competitive project-funding on researchers' publication outputs. Using detailed information on applicants at the Swiss National Science Foundation (SNSF) and their proposals' evaluation, we employ a case-control design that accounts for individual heterogeneity of researchers and selection into treatment (e.g. funding). We estimate the impact of grant award on a set of output indicators measuring the creation of new research results (the number of peer-reviewed articles), its relevance (number of citations and relative citation ratios), as well as its accessibility and dissemination as measured by the publication of preprints and by altmetrics. The results show that the funding program facilitates the publication and dissemination of additional research amounting to about one additional article in each of the three years following the grant. The higher citation metrics and altmetrics of publications by funded researchers suggest that impact goes beyond quantity, but that funding fosters quality and impact.

==> Neuer Ordner/latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> latexmkrc.tex <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
